An End-to-End Network Pruning Pipeline with Sparsity Enforcement

Neural networks have emerged as a powerful tool for solving complex tasks across various domains, but their increasing size and computational requirements have posed significant challenges in deploying them on resource-constrained devices. Neural network sparsification, and in particular pruning, has emerged as an effective technique to alleviate these challenges by reducing model size, computational complexity, and memory footprint while maintaining competitive performance. However, many pruning pipelines modify the standard training pipeline at only a single stage, if at all. In this work, we look to develop an end-to-end training pipeline that befits neural network pruning and sparsification at all stages of training. To do so, we make use of nonstandard model parameter initialization, pre-pruning training methodologies, and post-pruning training optimizations. We conduct experiments utilizing combinations of these methods, in addition to different techniques used in the pruning step, and find that our combined pipeline can achieve significant gains over current state of the art approaches to neural network sparsification.

==> sections/experiments.tex <==
\section{Experiments}

\begin{table*}[ht]
\small
\centering
\begin{tabular}{lccccccc}
    \toprule
    Dataset & Architecture & Rand & Mag & SNIP & GraSP & SynFlow & Butterfly + K-Matrix  \\
    \midrule
    CIFAR-10 & VGG16 & 10.00 & \underline{87.36} & 73.21 & 29.17 & 79.75 & \textbf{88.01}\\
    MNIST & FC & 94.49 & \textbf{97.57} & 95.54 & 94.74 & 11.35 & \underline{96.49} \\
    \midrule
    \textit{Butterfly head} \\
    CIFAR-10 & VGG16 & 10.00 & 10.00 & 86.52 & 14.04 & \underline{87.47} & \textbf{88.12} \\
    MNIST & FC & 94.84 & \underline{97.25} & 96.00 & 94.63 & 11.35 & \textbf{97.44} \\
    \bottomrule
\end{tabular}
\caption{Reported top-1 accuracies on MNIST and CIFAR-10 for pruning methods with sparsity $0.1$. In the bottom half of the table, the final classification head is a Butterfly matrix. In the column Butterfly + K matrix, instead of applying pruning, the entire model is replaced with Butterfly matrices for linear layers and K matrices for 2D convolutional layers. Each model was trained for $50$ epochs post-pruning, and the Mag pruning model was also pre-trained for $10$ epochs.}
\label{tab:1}
\end{table*}

\subsection{Fixing the sparsity at 0.1 and adding butterfly matrices} 
Mimicking the experiments from the Pruning assignment, the following results are reported for test accuracy (top 1) on either CIFAR-10 or MNIST with $10^{-1}$ sparsity in Table \ref{tab:1}. In addition to evaluating the pruning methods, we evaluate the replacement of all fully-connected layers in either the FC or VGG16 models, and also the replacement of just the final head with additional pruning. Noticably, introducing Butterfly matrices at the classification head does affect whether pruning method exhibits layer collapse early on, specifically in the case of Magnitude pruning, and replacing each layer with a butterfly/Kaleidoscope matrix generally yields better accuracy, although at the cost of higher inference times. The higher inference times are most likely due to an inefficiencies in the implemented Butterfly matrix multiplication kernel, which can potentially be fixed.

% Notably, SynFlow collapses on the fully-connected model on MNIST and the random model collapses on VGG16. Additionally, the performance of GraSP is generally worse than the other models, and this can potentially be explained by the fact that GraSP is motivated by the neural tangent kernel (NTK) which approximates better for wider networks. However, VGG16 and the fully-connected network are both not very wide, which may explain the dip in performance. As for SynFlow, it was never explicitly tested on MNIST in the original paper, and potentially for a fully-connected layer it requires extra tuning to work properly. It should be noted that all experiments were run with roughly the same hyperparameters, and therefore if some methods require some tuning, their performance may be worse here. 

\subsection{Effects of Aggressive Pruning with Factorized Prediction Heads}
Following the structure of the pruning assignment, we closely investigate the effects of changing the sparsity on VGG16 applied to the CIFAR-10 dataset. Based on sparsity values in $\{0.05,0.1,0.2,0.5,1,2\}$, we look at how the replacement of prunable layers with sparse butterfly factorizations affects the inference speed, accuracy, and overall FLOPS sparsity of the models. 

\begin{table*}[ht]
\small
\centering
\begin{tabular}{lcccccc}
    \toprule
    Sparsity & Rand & Mag & SNIP & GraSP & SynFlow & Butterfly + K-Matrix \\
    \midrule
    \textit{Butterfly matrix class-head} \\
    0.05 & \textbf{1.67} & 1.72 & 1.71 & 1.701 & 1.782 & 77.11 \\
    0.1 & \textbf{1.66} & 1.74 & 1.73 & 1.703 & 1.957 & - \\
    0.2 & 1.68 & 1.68 & 1.70 & 1.68 & \textbf{1.6659} & - \\
    0.5 & \textbf{1.667} & 1.67 & 1.69 & 1.70 & 1.71 & - \\
    1 & \textbf{1.628} & 1.63 & 1.66 & 1.71 & 1.71 & -\\
    2 & 1.642 & 1.68 & 1.66 & \textbf{1.60} & 1.663 & - \\
    \midrule
    0.05 & 1.672 & 1.721 & \textbf{1.62} & 1.71 & 1.68 & 75.02\\
    0.1 & 1.656 & 1.729 & \textbf{1.61} & 1.66 & 1.65 & 74.61 \\
    0.2 & 1.69 & 1.677 & \textbf{1.59} & 1.647 & 1.685 & 76.82 \\
    0.5 & 1.67 & 1.69 & \textbf{1.62} & 1.66 & 1.68 & 75.23 \\
    1 & 1.629 & 1.689 & 1.64 & \textbf{1.595} & 1.693 & 75.20 \\
    2 & \textbf{1.546} & 1.692 & 1.70 & 1.64 & 1.669 & 75.59 \\
    \bottomrule
\end{tabular}
\caption{Reported inference speed \textbf{in seconds} for VGG-16 running on CIFAR-10. The bottom half of the table uses a prunable dense classification head, while the top half uses a butterfly matrix as the classification head. For Butterfly + K-Matrix, all 2D convolutional layers in VGG16 are replaced with a Kaleidoscope-matrix implementation of 2D convolutions. When using a Butterfly matrix head and K-matrices, the model is not iteratively prunable. Additionally, the extremely slow inference time is most likely due to inefficiencies in the SpMV implementation for these 2D convolution operations. }
\label{tab:speed}
\end{table*}

\paragraph{Effect on Inference Speeds}
In \cite{dao2020learning}, they suggest that Butterfly matrices are a more structured and well-behaved version of pruning. However, the results presented in Table \ref{tab:speed} are quite interesting, as they suggest actually that most pre-initialization pruning methods do not pair well with an already-pruned classification head. Additionally, magnitude-based pruning, which performs weight thresholding by pre-training on the data, has a $\approx 5 \times$ inference speed slow-down with the introduction of a single Butterfly matrix layer head under the same hyperparameters as the original Pruning assignment, and the model itself actually completely collapses if pre-training for too long. A potential explanation is that magnitude-based pruning, which tries to keep the last layer dense based on heuristics, fails when the last layer is inherently not dense.

For the rest of the pruning methods, generally it is observed that introducing a Butterfly-matrix classification head does not affect inference speeds much. Any minor differences in speeds is generally a result of noise, as there is no perceivable pattern between sparsity and inference speeds when comparing the use of a prunable dense classification head and a Butterfly matrix.

Finally, when replacing the entire VGG-16 model with K-matrices, it is observed that the model inference speed is significantly slower. I suspect that this is an issue with the implementation of the SpMV kernel for Butterfly matrices and the implementation \cite{dao2020learning, dao2021kaleidoscope} use for \texttt{KOPS2D} layers, which are the drop-in replacement of 2D convolutional layers with K-matrices. For completion sake the numbers were kept in, but they do not offer useful analysis for the relationship between pruning and Butterfly matrices.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/acc_BH.png}
    \caption{For sparsity $10^{-k}$ for $k \in {0.05,0.1,0.2,0.5,1,2}$, the plot shows the top-1 accuracy of VGG-16 on CIFAR-10 for each pruning method using either a dense classification head or a Butterfly matrix head (labelled as + BH and with dashed lines). Generally, the introduction of the Butterfly matrix head degrades the performance of all pruning methods, most likely due to incompatability between the pruning metric and the fact that the Butterfly Matrix can be considered "already pruned".}
    \label{fig:accuracy}
\end{figure}

\paragraph{Effect on Model Accuracy} The effects of pruning and the use of Butterfly-matrix classification heads on accuracy of VGG-16 on CIFAR-10 are summarized in \ref{fig:accuracy}. 

Without considering the Butterfly matrix classification heads, GraSP notably performs poorly in the given setup, and there is an observable high variance in performance, although it generally performs worse than every other method. Additionally, SynFlow suffers from layer collapse despite its design to combat layer collapse, although this is most likely a a hyperparameter tuning issue because they report different results in their own paper. Only SNIP shows a small degradation in performance as sparsity increases with the overall model performance being strong.

The introduction of the Butterfly matrix head significantly degrades the performance of many of the pruning methods and even leads to faster layer collapse. Firstly, every evaluated pruning method collapses for sparsity $10^{-2}$. In the case of magnitude-based pruning, when using the hyperparameters specified in the original Pruning assignment (200 pre-training epochs and 100 post-training epochs), the model always collapses no matter what the sparsity is set to. This observation is related to the inference time slow-downs discussed in the previous section, although the exact reasoning is a bit unclear. For random pruning and SynFlow, the introduction of the Butterfly head does not affect the overall accuracy much: generally, either method exhibits layer collapse with a prunable dense classification head if and only if it exhibits layer collapse with a Butterfly matrix classification head. However, SNIP and GraSP both show significant degradations in performance, with SNIP only showing layer collapse with the introduction of the Butterfly matrix classification head. 

Finally, it is notable that from Table \ref{tab:1}, while replacing all VGG-16 layers with Butterfly/K-matrices significantly increases inference time, the overall accuracy is similar in performance to a base VGG-16. However, this is not that surprising, considering the sparsity introduced by factorized matrices is far less than that of the iterative pruning methods used.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/total_flops.png}
    \caption{For sparsity $10^{-k}$ for $k \in {0.05,0.1,0.2,0.5,1,2}$, this plot shows the FLOPS sparsity for each pruning method with and without the Butterfly layer head applied to VGG16 on CIFAR-10. Notably, the introduction of the Butterfly head generally increases the FLOPS sparsity by a marginal amount because the Butterfly layer head is not prunable, except for methods like random pruning and SynFlow that explicitly prune a certain percentage of the weights.}
    \label{fig:flop_total}
\end{figure}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/flops_bh.png}
    \caption{For sparsity $10^{0.5}$, this plot shows the FLOPS sparsity of each layer for each pruning method with and without the Butterfly layer head applied to VGG16 on CIFAR-10.}
    \label{fig:flops_layer}
\end{figure}

\paragraph{Effect on FLOPS Sparsity} The results are shown in Figures \ref{fig:flop_total} and \ref{fig:flops_layer}. Quite unsurprisingly, the effect of introducing a single Butterfly matrix head with the pruning methods does not affect FLOPS sparsity that much, although it is generally slightly higher overall and per layer. Additionally, we note that most layers tend to prune quite aggressively for deeper layers in the network, and across all methods, generally the layer right before the classification head is more aggressively pruned if the final classification head is a Butterfly matrix. 

Overall, the structure of VGG-16 is to increase in model parameters as the model gets deeper except for the prediction head, and all pruning methods other than random pruning will prune a higher percentage of these layers as expected. Additionally, SynFlow is the most conservative in pruning earlier smaller layers as expected to prevent bottlenecks, but heavily prunes the larger layers. Magnitude-based pruning has the staircase effect as described in the SynFlow paper, which is due to layer pruning at different rates. 

==> sections/fixed_sparsity.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{lccccccc}
    \toprule
    Dataset & Architecture & Rand & Mag & SNIP & GraSP & SynFlow & None  \\
    \midrule
    CIFAR-10 & VGG16 & 10.00 & 87.36 & 73.21 & 29.17 & 79.75 & - \\
    MNIST & FC & 94.49 & 97.57 & 95.54 & 94.74 & 11.35 & 97.66 \\
    \midrule
    \textit{Replace nn.Linear with Butterfly} \\
    CIFAR-10 & VGG16 & - & - & - & - & - & - \\
    MNIST & FC & - & - & - & - & 11.35 & 97.44 \\
    \bottomrule
\end{tabular}
\caption{}
\label{tab:1}
\end{table*}

==> sections/method.tex <==
\section{Method}
In this paper, we explore the effects of interspersing existing pruning methods and matrix factorization methods on image classification networks. In particular, we investigate whether applying a mixture of sparse-factorized layers and pruning to dense layers leads to any differences in speed-ups, as well as potential layer collapse issues. We specifically focus on factorizing just the final classification head or factorizing all layers in the model, and we only apply pruning methods to the dense layers.

\subsection{Methods of Introducing Sparsity}
We explore $5$ pruning methods, namely random pruning, magnitude-based pruning, SNIP, GraSP, and SynFlow, as well as $2$ sparse matrix factorization methods, namely Butterfly matrix decomposition for fully-connected layers and Kaleidoscope or K-matrix decomposition for 2D convolutional layers. Notably, other than magnitude-based pruning, the examined pruning methods prune an untrained model on initialization based on a variety of metrics that also influence which layers/neurons tend to get aggressively pruned. When introducing layers composed of the product of several structured low-rank matrices, it is interesting to investigate which pruning methods begin to suffer from layer collapse.

\subsection{Base Model Architectures}
Similar to the pruning assignment, we use a simple MLP classifier that consists of $L=6$ linear layers with a ReLU non-linearity for the MNIST dataset, and VGG16 on the CIFAR-10 dataset. In our experiments, we either replace the final classification head of the MLP or VGG16 with a butterfly-factorized linear layer, or every linear layer with a butterfly-factorized linear layer. In the case of VGG16, we replace 2D convolutional layers with an equivalent K-matrix representation. All experiments use a learning rate of $0.001$, a drop-out rate of $0.1$ on all layers, a batch-size of $256$, and the Adam optimizer with default settings. All experiments were run on a single NVIDIA GeForce RTX 3090.

\subsection{Choice of Factorization Layers}
The implementation of the Butterfly matrices and Kaleidoscope matrices makes it difficult to explicitly prune. Additionally, because \cite{dao2020learning, dao2021kaleidoscope} meant for Butterfly matrices to be a principled way to perform pruning, it was strange to perform an additional pruning step on these layers. Thus, all Butterfly/K-matrix layers are explicitly not pruned using the methods presented. Additionally, we focus on introducing Butterfly matrices either at the classification head or throughout the entire network to test whether introducing low-rank maps at the final step introduces any bottlenecks with evaluated the pruning methods.

==> sections/setup.tex <==
\usepackage[left=20mm,right=20mm,top=30mm,bottom=23mm,
head=30mm, headsep=3mm, foot=6mm, footnotesep=3mm,
includefoot]{geometry}

\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    urlcolor=orange,
    citecolor=teal,
}
\usepackage{fancyhdr}
\ctexset{%
    abstractname = \zihao{-3}Abstract,
    bibname = References,
    figurename = Figure,
    tablename = Table,
    section = {%
        fixskip     = true,
        beforeskip  = 7mm,
        indent      = 0pt,
        format      = \zihao{-3}\bfseries\centering,
        afterindent = true,
        aftername   = ~,
        afterskip   = 7mm,
    },
    subsection = {%
        fixskip     = true,
        beforeskip  = 6mm,
        indent      = 0pt,
        format      = \zihao{4}\bfseries,
        afterindent = true,
        aftername   = ~,
        afterskip   = 6mm,
    },
    paragraph = {%
        fixskip     = true,
        afterindent = true,
    },
}
\linespread{1.5}

\setmainfont{Times New Roman}
\setmathrm{Times New Roman}
\setCJKmathfont{Times New Roman}

\newcommand{\apj}{The Astrophysical Journal}
\newcommand{\apjl}{The Astrophysical Journal Letters}
\newcommand{\apjs}{Astrophysical Journal Supplement}
\newcommand{\aap}{Astronomy \& Astrophysics}
\newcommand{\nat}{Nature}
\newcommand{\araa}{Annual Review of Astronomy and Astrophysics}
\newcommand{\mnras}{Monthly Notices of the Royal Astronomical Society}
\newcommand{\jcap}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\prl}{Physical Review Letters}
\newcommand{\prd}{Physical Review D}
\newcommand{\eprint}[1]{\url{https://arxiv.org/abs/#1}}
\newcommand{\dd}{\mathrm{d}}

\AtBeginDocument{%
    \renewcommand{\ref}[1]{\autoref{#1}}
    \def\equationautorefname~#1\null{Equation~(#1)\null}
}
